Radiofrequency Ice Dielectric Measurements at Summit Station, Greenland

We recently reported on the radio-frequency attenuation length of cold polar ice at Summit Station, Greenland, based on bistatic radar measurements of radio-frequency bedrock echo strengths taken during the summer of 2021. Those data also include echoes attributed to stratified impurities or dielectric discontinuities within the ice sheet (layers), which allow studies of a) estimation of the relative contribution of coherent (discrete layers, e.g.) vs. incoherent (bulk volumetric, e.g.) scattering, b) the magnitude of internal layer reflection coefficients, c) limits on the azimuthal asymmetry of reflections (birefringence), and d) limits on signal dispersion in-ice over a bandwidth of ~100 MHz. We find that i) after averaging 10000 echo triggers, reflected signal observable over the thermal floor (to depths of approximately 1500 m) are consistent with being entirely coherent, ii) internal layer reflection coefficients are measured at approximately -60 to -70 dB, iii) birefringent effects for vertically propagating signals are smaller by an order of magnitude relative to comparable studies performed at South Pole, and iv) within our experimental limits, glacial ice is non-dispersive over the frequency band relevant for neutrino detection experiments.

==> author_list.tex <==
\author[Aguilar and others]{
J.~A.~Aguilar$^{1}$,
P.~Allison$^{2}$,
J.~J.~Beatty$^{2}$,
D.~Besson$^{3,4}$,
A.~Bishop$^{5}$,
O.~Botner$^{6}$,
S.~Bouma$^{7}$,
S.~Buitink$^{8}$,
M.~Cataldo$^{7}$,
B.~A.~Clark$^{9}$,
Z.~Curtis-Ginsberg$^{10}$,
A.~Connolly$^{2}$,
P.~Dasgupta$^{1}$,
S.~de Kockere$^{11}$,
K.~D.~de Vries$^{11}$,
C.~Deaconu$^{10}$,
M.~A.~DuVernois$^{5}$,
C.~Glaser$^{6}$,
A.~Hallgren$^{6}$,
S.~Hallmann$^{12}$,
J.~C.~Hanson$^{23}$,
B.~Hendricks$^{14}$,
C.~Hornhuber$^{3}$,
K.~Hughes$^{10}$,
A.~Karle$^{5}$,
J.~L.~Kelley$^{5}$,
I.~Kravchenko$^{15}$,
R.~Krebs$^{14}$,
R.~Lahmann$^{7}$,
U.~Latif$^{11}$,
J.~Mammo$^{15}$,
Z.~S.~Meyers$^{12,7}$,
K.~Michaels$^{10}$,
K.~Mulrey$^{16}$,
A.~Nelles$^{12,7}$,
A.~Novikov$^{3}$,
A.~Nozdrina$^{3}$,
E.~Oberla$^{10}$,
B.~Oeyen$^{17}$,
Y.~Pan$^{18}$,
H.~Pandya$^{8}$,
I.~Plaisier$^{7,12}$,
N.~Punsuebsay$^{18}$,
L.~Pyras$^{12,7}$,
D.~Ryckbosch$^{17}$,
O.~Scholten$^{11,19}$,
D.~Seckel$^{18}$,
M.~F.~H.~Seikh$^{3}$,
D.~Smith\thanks{e-mail: danielsmith@uchicago.edu, authors@rno-g.org}$^{~,10}$,
D.~Southall$^{10}$,
J.~Torres$^{2}$,
S.~Toscano$^{1}$,
D.~Tosi$^{5}$,
D.~J.~Van Den Broeck$^{11,8}$,
N.~van Eijndhoven$^{11}$,
A.~G.~Vieregg$^{10}$,
C.~Welling$^{7,12}$,
D.~R.~Williams$^{20}$,
S.~Wissel$^{14,21}$,
R.~Young$^{3}$,
A.~Zink$^{7}$
}
\affiliation{
$^{1}$Universit\'e Libre de Bruxelles, Science Faculty CP230, B-1050 Brussels, Belgium\\
$^{2}$Dept. of Physics, Center for Cosmology and AstroParticle Physics, Ohio State University, Columbus, OH 43210, USA\\
$^{3}$University of Kansas, Dept.~of Physics and Astronomy, Lawrence, KS 66045, USA\\
$^{4}$National Nuclear Research University MEPhI, Kashirskoe Shosse 31, 115409, Moscow, Russia\\
$^{5}$Wisconsin IceCube Particle Astrophysics Center (WIPAC) and Dept.~of Physics, \\ University of Wisconsin-Madison, Madison, WI 53703,  USA\\
$^{6}$Uppsala University, Dept.~of Physics and Astronomy, Uppsala, SE-752 37, Sweden\\
$^{7}$Erlangen Center for Astroparticle Physics (ECAP), \\  Friedrich-Alexander-University Erlangen-Nuremberg, 91058 Erlangen, Germany\\
$^{8}$Vrije Universiteit Brussel, Astrophysical Institute, Pleinlaan 2, 1050 Brussels, Belgium\\
$^{9}$Dept.~of Physics and Astronomy, Michigan State University, East Lansing MI 48824, USA\\
$^{10}$Dept.~of Physics, Enrico Fermi Inst., Kavli Inst.~for Cosmological Physics, University of Chicago, Chicago, IL 60637, USA\\
$^{11}$Vrije Universiteit Brussel, Dienst ELEM, B-1050 Brussels, Belgium\\
$^{12}$DESY, Platanenallee 6, 15738 Zeuthen, Germany\\
$^{13}$Whittier College, Whittier, CA 90602, USA\\
$^{14}$Dept.~of Physics, Dept.~of Astronomy \& Astrophysics, Penn State University, University Park, PA 16801, USA\\
$^{15}$Dept.~of Physics and Astronomy, Univ.~of Nebraska-Lincoln, NE, 68588, USA\\
$^{16}$Department of Astrophysics/IMAPP, Radboud University, PO Box 9010, 6500 GL, The Netherlands\\
$^{17}$Ghent University, Dept. of Physics and Astronomy, B-9000 Gent, Belgium\\
$^{18}$Dept.~of Physics and Astronomy, University of Delaware, Newark, DE 19716, USA\\
$^{19}$Kapteijn Institute, University of Groningen, Groningen, The Netherlands\\
$^{20}$Dept.\ of Physics and Astronomy, University of Alabama, Tuscaloosa, AL 35487, USA\\
$^{21}$Physics Dept. California Polytechnic State University, San Luis Obispo CA 93407, USA\\
}

